Hard X-ray luminosity function and absorption distribution of nearby AGN: INTEGRAL all-sky survey

We use the INTEGRAL all-sky hard X-ray survey to perform a statistical study of a representative sample of nearby AGN. Our entire all-sky sample consists of 127 AGN, of which 91 are confidently detected (>5 sigma) on the time-averaged map obtained with the IBIS/ISGRI instrument and 36 are detected only during single observations. Among the former there are 66 non-blazar AGN located at |b|>5 deg, where the survey's identification completeness is ~93%, which we use for calculating the AGN luminosity function and X-ray absorption distribution. In broad agreement with previous studies, we find that the fraction of obscured (log NH>22) objects is much higher (~70%) among the low-luminosity AGN (Lx<10^43.6 erg/s) than among the high-luminosity ones (Lx>10^43.6 erg/s), \~25%, where Lx is the luminosity in the 17-60 keV energy band. We also find that locally the fraction of Compton-thick AGN is less than 20% unless there is a significant population of AGN that are so strongly obscured that their observed hard X-ray luminosities fall below 10^40-10^41 erg/s, the effective limit of our survey. The constructed hard X-ray luminosity function has a canonical, smoothly broken power-law shape in the range 40<log Lx<45.5 with a characteristic luminosity of log L*=43.40+/-0.28. The estimated local luminosity density due to AGN with log Lx>40 is (1.4+/-0.3) 10^39 erg/s/Mpc^3 (17-60 keV). We demonstrate that the spectral shape and amplitude of the CXB are consistent with the simple scenario in which the NH distribution of AGN (for a given Lx/L*(z) ratio has not changed significantly since z~1.5, while the AGN luminosity function has experienced pure luminosity evolution.

==> agn_sl5_table.tex <==
\begin{table*}
\caption{INTEGRAL all-sky survey AGN sample
}
\smallskip

\scriptsize

\begin{tabular}{lcrrrrrcr}
\hline
\hline
\multicolumn{1}{c}{Source$^{\rm a}$} &
\multicolumn{1}{c}{Class$^{\rm b}$} &
\multicolumn{1}{c}{$z$} &
\multicolumn{1}{c}{$D$} &
\multicolumn{1}{c}{Note$^{\rm c}$} &
\multicolumn{1}{c}{$F_{\rm 17-60~keV}$} & 
\multicolumn{1}{c}{$\log L_{\rm hx}$} &
\multicolumn{1}{c}{$N_{\rm H}$} & 
\multicolumn{1}{c}{Ref$^{\rm d}$} \\
   
\multicolumn{1}{c}{} &     
\multicolumn{1}{c}{} &     
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{Mpc} & 
\multicolumn{1}{c}{} &     
\multicolumn{1}{c}{10$^{-11}$~erg/s/cm$^{2}$} &       
\multicolumn{1}{c}{erg/s} &     
\multicolumn{1}{c}{10$^{22}$cm$^{-2}$} &
\multicolumn{1}{c}{} \\
\hline
NGC 0526A                       &  S1.5 &  0.0191 &       &  & $3.72\pm0.97$ &  43.43 & & \\
ESO 297-G018                    &  S2   &  0.0252 &       &  & $4.41\pm0.94$ &  43.75 & & \\
NGC 1052                        &  S2   &  0.0050 &  17.8 &  & $2.12\pm0.43$ &  41.91 & & \\
{\bf LEDA 168563}               &  S1   &  0.0290 &       &  & $4.42\pm1.11$ &  43.88 & & \\
AKN 120                         &  S1   &  0.0327 &       &  & $8.38\pm3.52$ &  44.26 & & \\
MCG 8-11-11                     &  S1.5 &  0.0205 &       &  & $5.61\pm1.51$ &  43.67 & & \\ 
{\bf IRAS 05589+2828}           &  S1   &  0.0330 &       &  & $3.03\pm0.62$ &  43.83 & & \\ 
PG 0804+761                     &  S1   &  0.1000 &       &  & $1.21\pm0.33$ &  44.43 & & \\ 
NGC 4051                        &  S1.5 &  0.0023 &  17.0 &  & $2.11\pm0.54$ &  41.87 & & \\
NGC 4138                        &  S1.9 &  0.0030 &  17.0 &  & $2.39\pm0.49$ &  41.92 & & \\
WAS 49B                         &  S2   &  0.0630 &       &  & $0.95\pm0.35$ &  43.91 & & \\ 
NGC 4253                        &  S1.5 &  0.0129 &       &  & $1.53\pm0.31$ &  42.70 & & \\
NGC 4258                        &  S1.9 &  0.0015 &   6.8 &  & $1.90\pm0.56$ &  41.03 & & \\ 
XSS J12389-1614=IGR J12391-1612 &  S2   &  0.0367 &       &20& $3.01\pm0.62$ &  43.92 & & \\ 
{\bf WKK 1263}                  &  S2   &  0.0244 &       &  & $1.28\pm0.31$ &  43.19 & & \\ 
PKS 1241-399                    &  QSO  &  0.1910 &       &  & $1.77\pm0.40$ &  45.21 & & \\ 
Mrk 783                         &  S1.5 &  0.0672 &       &  & $1.23\pm0.32$ &  44.08 & & \\ 
NGC 5033                        &  S1.9 &  0.0029 &  18.7 &  & $1.21\pm0.28$ &  41.71 & & \\ 
ESO 383-G018                    &  S2   &  0.0124 &       &  & $1.74\pm0.38$ &  42.72 & & \\ 
NGC 5252                        &  S1.9 &  0.0230 &       &  & $2.60\pm0.78$ &  43.44 & & \\ 
NGC 5548                        &  S1.5 &  0.0172 &       &  & $2.06\pm0.50$ &  43.08 & & \\ 
ESO 511-G030                    &  S1   &  0.0224 &       &  & $3.33\pm0.91$ &  43.53 & & \\ 
NGC 6240                        &  S2   &  0.0245 &       &  & $4.66\pm1.38$ &  43.75 & & \\
3C 382                          &  S1   &  0.0579 &       &  & $3.96\pm1.75$ &  44.45 & & \\ 
ESO 103-G035                    &  S2   &  0.0133 &       &  & $6.64\pm1.34$ &  43.37 & & \\
XSS J19459+4508=IGR J19473+4452 &  S2   &  0.0532 &       &21& $1.52\pm0.45$ &  43.96 & & \\
3C 403                          &  NLRG &  0.0590 &       &  & $0.96\pm0.33$ &  43.85 & & \\
4C +74.26                       &  BLRG &  0.1040 &       &  & $3.93\pm1.22$ &  44.98 & & \\ 
S5 2116+81                      &  S1   &  0.0840 &       &  & $2.91\pm0.98$ &  44.65 & & \\ 
NGC 7314                        &  S1.9 &  0.0048 &       &  & $2.17\pm0.58$ &  41.99 & & \\ 

\end{tabular}

$^{\rm c}$ Note or reference for INTEGRAL discovered AGN: (20) =2MASX
J12390630-1610472 \citep{sazetal05,masetal06}, (21) =2MASX
J19471938+4449425 \citep{sazetal05,biketal06,masetal06b}

\end{table*}

